On the Expressive Power of Geometric Graph Neural Networks

The expressive power of Graph Neural Networks (GNNs) has been studied extensively through the Weisfeiler-Leman (WL) graph isomorphism test. However, standard GNNs and the WL framework are inapplicable for geometric graphs embedded in Euclidean space, such as biomolecules, materials, and other physical systems. In this work, we propose a geometric version of the WL test (GWL) for discriminating geometric graphs while respecting the underlying physical symmetries: permutations, rotation, reflection, and translation. We use GWL to characterise the expressive power of geometric GNNs that are invariant or equivariant to physical symmetries in terms of distinguishing geometric graphs. GWL unpacks how key design choices influence geometric GNN expressivity: (1) Invariant layers have limited expressivity as they cannot distinguish one-hop identical geometric graphs; (2) Equivariant layers distinguish a larger class of graphs by propagating geometric information beyond local neighbourhoods; (3) Higher order tensors and scalarisation enable maximally powerful geometric GNNs; and (4) GWL's discrimination-based perspective is equivalent to universal approximation. Synthetic experiments supplementing our results are available at \url{https://github.com/chaitjo/geometric-gnn-dojo}

==> tex/complexity.tex <==
\section{Time and Space Complexity of GWL}
\label{app:complexity}

At present, we consider GWL as an abstract mathematical tool for uncovering practical results about geometric GNN models rather than an efficiently implementable algorithm. 
This is because both GWL and WL assume perfect hash functions, which may require infinite space complexity in general, such as when using an infinite-order spherical harmonics expansion Therefore, implementing these methods efficiently can be challenging.

We provide a preliminary analysis of the time and space complexity of GWL.
\begin{itemize}
    \item Let $v$ be the number of nodes, $e$ the number of edges, and $d$ the maximum degree.
    \item Assume that the time and space complexity of $\textsc{I-Hash}$ is a function of the maximum degree and number of iterations, or alternatively a function of the number of nodes, as the largest neighbourhood that can occur will be of the order of magnitude of the entire set of nodes. Thus, we assume that the time and space complexity of $\textsc{I-Hash}$ is $\mathcal{O}(f(d, t))$ or $\mathcal{O}(f(v))$ in the limit.
    \item The time complexity of $t$ iterations of GWL is $\mathcal{O}(te + v f(d, t))$, as each iteration essentially performs message passing, which is $\mathcal{O}(te)$, followed by one application of $\textsc{I-Hash}$ per node, which is $\mathcal{O}(f(d, t))$ each.
    \item The space complexity of $t$ iterations of GWL is $\mathcal{O}(vd^t)$, as each node stores its $t$-hop subgraph at iteration $t$.
\end{itemize}



==> tex/gwl_for_so2.tex <==
\section{Alternative GWL formulation for $SO(2)$} 
\label{sec:gwl-so2}

\paragraph{Overview.} The version of GWL presented in the main text uses a geometric neighbourhood object $\vg$ that keeps increasing in size at each iteration. A natural question to ask is whether a more fixed-length encoding of the neighbourhood's orientation can be obtained. In this section, we show this is possible for $SO(2)$, which has some particularly convenient properties: it is commutative, and its (discrete) subgroups are particularly simple. 
% First, we point out why, when working with the standard representation of $SO(d)$ acting on vectors in $\sR^d$, the orientation of a neighbourhood cannot be (injectively) encoded into another vector obtained from permutation invariant aggregation. 

\begin{definition}[Representation]
A representation of a group $\fG$ on a vector space $V$ over is a group homomorphism from $\fG$ to $GL(V)$, the general linear group on $V$, i.e. a map $\rho: \fG \to GL(V)$ such that $\rho(\fg_1 \fg_2) = \rho(\fg_1) \rho(\fg_2)$. 
\end{definition}

Let $\mX \in \sR^{n \times d}$ be a point cloud of size $n$ in $\sR^d$ and denote by $\rho_0$ the standard representation of $\fG = SO(d)$. Then, one can show that there is no $S_n$-invariant, $\fG$-equivariant function that is injective over $\gO_\fG(\mX)$, i.e. the orbit of $\mX$. This is due to the presence of point clouds with discrete rotational symmetry (i.e. snowflake structures). This is shown in the next result. 

\begin{proposition}[The Discrete Symmetry Problem]
Let $\mX \in \sR^{n \times 2}$ be a point cloud with $n$ points having discrete rotational symmetry, i.e. there exists $\pi \in S_n$ and $\fg \neq \mathrm{id} \in O(2)$ s.t. $\pi\mX = \fg \mX$. Then, any permutation-invariant and $O(d)$-equivariant function $f: \sR^{n \times 2} \to \sR^2$ has the property that $f(\mX) = f(\fg \mX) = 0$ for all $\fg$. 
\end{proposition}

\begin{proof}
$\pi\mX = \fg\mX \implies f(\pi\mX) = f(\fg\mX) \implies f(\mX) = \rho^0(\fg)f(\mX) \implies f(\mX) = 0$

The last statement follows from the fact that the only fixed point of a 2D orthogonal matrix is the zero vector. This result easily extends to any dimension $d$ by finding a set of vectors that span a two-dimensional plane and performing a rotation in that plane. 
\end{proof}

% associated representations $\rho_1, \ldots, \rho_n: \fG \to SO(d)$. Furthermore assume that $\fG$ acts on $\sR^{n \times d}$ via $\fg\mX := [ \rho^1(\vx_1), \ldots, \rho^n(\vx_n) ]$. We want to find a multi-set function $f: \gX^n \to \sR^d$ that is $O(d)$-equivariant and injective over the orbit of $X$, denoted by $\gO_\fG(X)$. 

\paragraph{Implications.} The result shows that when a standard representation is used, it is impossible to injectively summarise the orientation of the point cloud in a vector that is independent of the size of the point cloud. To circumvent this issue, the GWL algorithm presented in the main text stores the entire neighbourhood around a node in order to understand its orientation. Next, we show that when an alternative group representation is used, we can faithfully aggregate the orientation of the neighbourhood in a 2D vector if $\fG = SO(2)$ and $d=2$. Therefore, from now on, we work in this setting. 

\begin{theorem}\label{theo:so2_gwl}
There exists a representation $\rho: \fG \to SO(\sR^2)$ and a multi-set function $\textsc{Hash}_{v}$ sending $X$ to $\sR^2 \setminus \{0\}$ that is unique for each multi-set $X \subset \gX$ of bounded size and $\textsc{Hash}_{v}(\fg X) = \rho(\fg)\textsc{Hash}_{v}(X)$. 
Furthermore, for any two $X_1, X_2 \subset \gX$ we have that $\norm{\textsc{Hash}_{v}(X_1)} = \norm{\textsc{Hash}_{v}(X_2)}$ iff there is $\fg \in \fG$ such that $gX_1 = X_2$.
\end{theorem}

\begin{proof}
Let $\gO_\fG(X)$ be an orbit of $X$ generated by the action of the group $\fG=SO(2)$ acting on $\sR^{n \times d}/S_n$ (i.e. the space of multi-sets of 2D vectors) as in the statement of Theorem \ref{theo:so2_gwl}. Then, $SO(2)$ acts transitively on $\gO_\fG(X)$ by construction. 
\begin{center}
\begin{tikzcd}
\gO_{\fG}(X) \arrow[r, "\phi_{X}"] & SO(2)/\fG(X) \arrow[r, "\eta"] & SO(\sR^2) \arrow[r, "\omega_\vu"] & S^1 \subset \sR^2 \\
& SO(2) \arrow[u, "\pi"] \arrow[ru, "\rho"] \arrow[rru, "\sigma_\vu"] & &
\end{tikzcd}
\end{center}
Denoting by $\fG(X)$ its isotropy/stabilizer group of $X$, the function $\phi_{X}: \gO(X) \to SO(2)/\fG(X)$ given by  $\phi_{X}(Y) = \phi_{X}(\fg X) = \fG(X)$ with $g \in SO(2)$ is well-defined and, moreover, it is an equivariant homeomorphism of $\fG$-spaces (\textit{e.g.} see Proposition 4.1 in \citet{bredon1972introduction}). 

Notice that because $SO(2)$ is abelian, $\fG(X)$ is a normal subgroup and $SO(2)/\fG(X)$ is not only a manifold, but also a (Lie) group. We will show that we can find a faithful orthogonal representation of this quotient group. Because we are working with finite neighbourhoods, the group $\fG(X)$ is a finite cyclic subgroup (standard result) if $X \neq 0$. Otherwise, $\fG(X) = SO(2)$. 

Therefore, let us denote by $\alpha(\fg \fG(X))$ the smallest angle of a rotation in the equivalence class $\fg \fG(X)$. If $\fG(X)$ is a finite cyclic subgroup generated by rotations of an angle $\theta$, then $\alpha(SO(2)/\fG(X)) = [0, \theta)$. If $\fG(X) = SO(2)$, then $\alpha(SO(2)/ \fG(X)) = 0$. Thus, we can construct the orthogonal representation $\eta: SO(2)/\fG(X) \to SO(\sR^d)$ given by $\eta(\fg\fG(X)) = \mR_{\alpha(SO(2)/\fG(X)) 2\pi/\theta}$ if $\fG(X)$ is finite and $\eta(\fg\fG(X)) = \mI$, otherwise. It can be checked that in either case, $\eta$ is an injective group homomorphism and, therefore, a faithful representation of the group.

Given $\vu = [1, 0] \in S^1 \subset R^2$, we can define a map $\omega_\vu: SO(\sR^d) \to S^1$ given by $\omega_\vu(\mR_\alpha) = \mR_\alpha \vu$, which is another homeomorphism. Thus, the composition is $\psi = \omega_\vu \circ \eta \circ \phi_X: \gO_{\fG}(X) \to \sR^2$ is an injective function. Moreover, because the quotient map $\pi: SO(2) \to SO(2)/\fG(X)$ is a group homomorphism, we can compose it with $\eta$ to lift the representation of $SO(2)/\fG(X)$ to a representation $\rho = \eta \circ \pi$ of $SO(2)$. Therefore, it follows that $\psi$ is also equivariant with respect to this representation of $SO(2)$. 

Finally, we can extend $\psi$ to a function that is injective for any multi-set by constructing a $\psi_{\gO_\fG(X)}$ for each orbit $\gO_\fG(X)$, where $X$ is a representative of the orbit, by using a map $\omega_{\gO_\fG(X)}$ where $\vu$ = $[\textsc{I-Hash}(X), 0]$ (i.e. the norm encodes the orbit).   
\end{proof}

% This allows us to define a Geometric Weisfeiler Lehman test for geometric graphs over $SO(2)$.

\textbf{Alternative $SO(2)$ Geometric Weisfeiler-Leman Test}. Given a geometric graph $(\gG, \mX, \mH)$, the $SO(2)$-GWL algorithm consists of three steps:
\begin{enumerate}
    \item For each node $v \in \gG$ and $u \in \gN(v)$, initialise:
    \begin{align}
        \vm_{v,u}^0 &:= \textsc{Hash}(\vh_v, \vh_u, \norm{\textsc{Hash}_{v}(\vx_v - \vx_u)}) \frac{\textsc{Hash}_{v}(\vx_v - \vx_u)}{\norm{\textsc{Hash}_{v}(\vx_v - \vx_u)}} \nonumber \\
        \vm_v^{0} &:= \textsc{Hash}_{v}(\vm_{v, u_1}^0, \ldots, \vm_{v, u_{d(v)}}^0) \nonumber
    \end{align}
    \item For each node $v \in \gG$, update $\vm_v^{l+1} := \textsc{Hash}_{v}(\vm_{u_1}^l, \ldots, \vm_{u_{d(v)}}^l)$. 
    \item Go back to step 2 until the partition induced by $\ldblbrace \norm{\vm_v^l} : v \in \gG \rdblbrace$ becomes stable.
    \item Return the colours of the nodes $\ldblbrace \norm{\vm_v^L} : v \in \gG \rdblbrace$ at the last iteration $L$.
\end{enumerate}

%%
